The $C_2$-effective spectral sequence for $C_2$-equivariant connective real $K$-theory

We construct a $C_2$-equivariant spectral sequence for RO$(C_2)$-graded homotopy groups. The construction is by using the motivic effective slice filtration and the $C_2$-equivariant Betti realization. We apply the spectral sequence to compute the RO$(C_2)$-graded homotopy groups of the completed $C_2$-equivariant connective real $K$-theory spectrum. The computation reproves the $C_2$-equivariant Adams spectral sequence results by Guillou, Hill, Isaksen and Ravenel.

==> ring.tex <==
\section{The homotopy ring \texorpdfstring{$\pi_{*,*}\ko$}{homotopy}}
\label{ring}

\begin{prop}
	The $(2,\eta)$-completed coweight $0$-stem of $\ko$ is 
	$$\Pi_0(\ko)\cong \bbZ_2[\eta,\rho,\alpha,\beta]/(\rho(\eta\rho+2),\eta(\eta\rho+2),\rho\alpha-\eta^3,\rho^3\beta-\eta\alpha,\alpha^2-4\beta),$$
	where the generators are in degrees:
	$$|\eta|=(1,1), ~~|\rho|=(-1,-1),~~|\alpha|=(4,4), ~~|\beta|=(8,8).$$
\end{prop}

\begin{proof}
	The generators are obtained by inspection the coweight $0$ $E_\infty$ page. The first two relation are in \ref{omegarelation}. The rest are \ref{alphadef} and \ref{alphabetarelation}.

\end{proof}

The result of $\pi_{*,*}^{C_2}(\ko^{\wedge}_{(\eta,2)})$ agrees with \cite{GHIR}. We refer to \cite[Section 11]{GHIR} for a complete description.

% copy paste?
